Dimensional Reweighting Graph Convolutional Networks

Graph Convolution Networks (GCNs) are becoming more and more popular for learning node representations on graphs. Though there exist various developments on sampling and aggregation to accelerate the training process and improve the performances, limited works focus on dealing with the dimensional information imbalance of node representations. To bridge the gap, we propose a method named Dimensional reweighting Graph Convolution Network (DrGCN). We theoretically prove that our DrGCN can guarantee to improve the stability of GCNs via mean field theory. Our dimensional reweighting method is very flexible and can be easily combined with most sampling and aggregation techniques for GCNs. Experimental results demonstrate its superior performances on several challenging transductive and inductive node classification benchmark datasets. Our DrGCN also outperforms existing models on an industrial-sized Alibaba recommendation dataset.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> paras/model.tex <==
\section{Dimensional Reweighting Module for GCNs}
%In this section, we introduce our dimensional reweighting block on graph convolutional networks, and how it can be combined with graph sampling and aggregation methods adaptively. 
\iffalse
\subsection{General GCN Framework}
We first introduce the general GCN framework as the background framework.  
Algorithm \ref{algo:gcn} shows a general graph convolutional layer. A graph convolutional layer generally transfers a set of node representations(features or hidden representations) on a graph to a set of refined node representations(hidden representations or embeddings) using neighborhood information of the graph. A graph convolutional layer involves three parts, the sampling procedure, the aggregation and the transformation procedure. The sampling producer samples a neighborhood for each node using a sampler, while the aggregation procedure aggregates sampled neighborhood information of the node. The sampler can be uniform \cite{hamilton2017inductive} or weighted\cite{chen2018fastgcn,huang2018adaptive}. The aggregator can be mean, LSTM \cite{hamilton2017inductive}, attention\cite{velivckovic2018graph} or gated attention\cite{zhang2018gaan}. The transformation procedure is usually a single-layer fully-connected neural network which can be separated to a linear matrix multiplication with bias added and an activation function. Commonly used activation functions include ELU, ReLU\cite{kipf2017semi,chen2018fastgcn,huang2018adaptive} and leaky-ReLU\cite{velivckovic2018graph}. It can also be other types of transformation functions as well such as the residual block\cite{velivckovic2018graph,he2016deep}.

Also, in some models, the transformation procedure can be splited by the aggregation procedure. These methods first do matrix multiplication with bias added, then aggregation, and finally activation. \cite{velivckovic2018graph} A full graph convolutional network is usually a stacking structure of graph convolutional layers where the first layer takes node features as input and all other layers takes the output of the pervious layer as input. Finally we use the output of the last layer for ndoe classification.
\fi
In this section, we detail the proposed dimensional reweighting module for GCNs. We first summarize the regular GCN layer in Algorithm \ref{algo:gcn}. 
%In this paper, we propose a \textbf{Dimension Reweighting} method, it basically adds a dimensional reweighting process before the neighborhood sampling, aggregation and transformation steps.
Given the node representations of the graph $\mathcal{R}_{i}$, our dimensional reweighting process tries to learn an adaptive scalar, which takes in a set of node embeddings in a hidden layer  $\mathcal{R}_i=\{\mathbf{r}^{i}_v|v\in\mathcal{V}\}$ and learns an adaptive scalar $\mathbf{s}=(s_1,...,s_d)$. The adaptive scalar reweighs each dimension for refined node representations $\{\mathbf{r}^{r}_v|v\in \mathcal{V}\}$, where $\mathbf{r}^{r}_v=\mathbf{s}*\mathbf{r}^{i}_v$ is the componentwise multiplication of $\mathbf{s}$ and $\mathbf{r}^{i}_{v}$. 
\begin{equation}
    r^{r}_{v,j}=s_jr^{i}_{v,j} ,\forall 1\leq j\leq d,\forall v\in\mathcal{V}.
\end{equation}
We call $\mathbf{s}$ a dimensional reweighting scalar. The dimensional reweighting graph convolutional layer is shown as algorithm \ref{algo:dr}. Inspired by SE-net\cite{hu2018squeeze}, we learn our dimensional reweighting scalar by first calculating the expected value of $\mathbf{r}^{i}$ and then applying an encoder-decoder structure. It first encodes information from different representations to a lower-dimensional representation $\mathbf{g}$, then decodes $\mathbf{g}$ to generate $\mathbf{s}$. Algorithm \ref{algo:drcom} denotes our method to generate the dimensional reweighting scalar $\mathbf{s}$.

\begin{algorithm}[t]
	\caption{Computation of Dimensional Reweighting Scalar \label{algo:drcom}}
	\KwIn{network $(\mathcal{V},\mathcal{E},\mathcal{R}_i)$, $\mathcal{V}$ set of nodes (in batch),$\mathcal{E}$ set of edges, $\mathcal{R}_i=\{\mathbf{r}^{i}_v|v\in \mathcal{V}\}$ set of input representations.  }
	\KwOut{dimensional reweighting scalar $\mathbf{s}$ }
	Generate node weights $\{w_v|v\in\mathcal{V}\}$, the weights shall satisfy $\sum_{v\in\mathcal{V}}w_v=1 ,\forall v,w_v\geq 0$
	
	Compute $\mathbf{r}^{i}=E[\mathbf{r}^{i}_v|v\in\mathcal{V}]=\sum_{v\in\mathcal{V}}w_v\mathbf{r}^{i}_{v}$
	
	Encode $\mathbf{r}^{i}$ with an encoder $\mathbf{g}=\sigma_g(\mathbf{W}_g\mathbf{r}^{i}+b_g)$
	
	Decode $\mathbf{g}$ to generate $\mathbf{s}$, $\mathbf{s}=\sigma_s(\mathbf{W}_s\mathbf{g}+b_s)$
	
	Output scalar $\mathbf{s}$
\end{algorithm}
\iffalse
\zc{Why do we need a lossy compressed g to reconstruct S, why there could be overffiting for such low dimension array, is this supported by the experiment? Do not introduce g until we are ready to show its necessity. }

Given $\mathbf{r^i}=E[\mathbf{r}^i_v|v\in\mathcal{V}]$, we then use this to form a lower-dimensional general representation $\mathbf{g}=(g_1,...g_r)$, where $r<<d$ is the lower-dimension encoded representation representing the scale of imbalance of weights on different representations.   Then we use this representation to construct a $d-$dimensional scalar $S=(s_1,...s_d)$. Finally, we do the embedding reweighting process,
\begin{equation}
v'_{i,j}=v_{i,j}s_j,\forall i,j
\end{equation}
\begin{equation}
    \mathbf{v'}_i=(v'_{i,1},...,v'_{i,d})^T, \forall i
\end{equation}

%\subsection{Weight of Nodes}
Series of recent discoveries points out that nodes in a graph do not always share the same importance. Weighted aggregation leads to better performance in GNN\cite{}, while weighted sampling does better than uniform sampling as well. \cite{} 

Theerfore, when being added on top of a weighted aggregation layer, in calculation of $v_{,j}=E[v_{i,j}|1\leq i\leq n]=\sum w_i v_{i,j}$, instead of assigning $w_i=\frac{1}{n}$ like what the original SE-net done for pixels in an image, we applies the importance of each node. Specifically, for attention based aggregation, the Attention-Reweight method is described as the following:

\begin{equation}
    v_{,j}=E[v_{i,j}|1\leq i\leq n]=\sum w_i v_{i,j},
\end{equation}
where $w_i$ is the expected attention weight of each node.
\begin{equation}
    w_i=mean(w_{j,i}|j\in\mathcal{G})
\end{equation}
where $w_{j,i}$ is the attention weight of edge $j\rightarrow i$
%\subsection{Calculation of Reweighting Scalars}
Once we get the expected value $\mathbf{v}=(\mathbf{v}_{,1},...,\mathbf{v}_{,d})^T$ of each representation using attention among the nodes on the graph, to prevent overfitting, we first encode such information to a low-dimensional space and form an encoded representation $\mathbf{g}$, then use $\mathbf{g}$ to generate a scalar $s$. Both of such operations uses a single layered fully-connected neural network as \cite{hu2018squeeze} did.
\begin{equation}
    \mathbf{g}=\sigma_{g}(\mathbf{W}_g\mathbf{v}+\mathbf{b}_g)
\end{equation}
\begin{equation}
    \mathbf{s}=\sigma_{s}(\mathbf{W}_s\mathbf{g}+\mathbf{b}_s)
\end{equation}
where $\mathbf{W}_g,\mathbf{W}_s$ are weights for the encoding and decoding process, and $\mathbf{b}_g,\mathbf{b}_s$ are biases. $\sigma_g$ and $\sigma_s$ are activation functions. $\sigma_g$ can be a simple activation function with non-linearity, such as $ReLU$ or $leaky-ReLU$, while as for $\sigma_s$, since $\mathbf{s}$ is used to scale $\mathbf{v}_i$, the value of $\mathbf{s}$ shall be around 1. So $\sigma_s$ shall be activation functions which do not produce values much larger than 1, therefore we choose $\sigma_s$ to be $sigmoid$.
\fi
%\subsection{Combination With Existing Graph Neural Network Methods}
Our dimensional reweighting method can be implemented as an independent functional process and easily combine with graph-based convolutional neural networks. As can shown in algorithm \ref{algo:dr}, our method does not coupling with any existing neighborhood sampling, neighborhood aggregation, or representation transformation methods. We'll further explain this in section \ref{sec:exp}, where we combine our $\textbf{DR}$ method with multiple existing sampling and aggregation GCN methods.

\begin{algorithm}[t]
	\caption{General Graph Convolutional Layer \label{algo:gcn}}
	\KwIn{network $(\mathcal{V},\mathcal{E},\mathcal{R}_i)$, $\mathcal{V}$ set of nodes (in batch),$\mathcal{E}$ set of edges, $\mathcal{R}_i=\{\mathbf{r}^{i}_v|v\in \mathcal{V}\}$ set of input representations.  }
	\KwOut{set of output representations $\mathcal{R}_o$ }
	
	\ForEach{$v\in \mathcal{V}$}{
	    Sample neighborhood $N_v\subseteq \mathcal{N}_v$\\
        Aggregate node representations of $N_v$ for node $v$ 
        $\mathbf{r}^{a}_v=a(\mathbf{r}^{i}_{t}|t\in N_v\cup \{v\})$\\
	    Use a neural network layer to transform $\mathbf{r}^{a}_v$ to output representation $\mathbf{r}_{v}^{o}$,      $\mathbf{r}_{v}^{o}=f(\mathbf{r}^{a}_{v})$ (Typically $f(\mathbf{x})=\sigma(\mathbf{W}\mathbf{x}+\mathbf{b})$)
	}
	Output $\mathcal{R}_{o}=\{\mathbf{r}_{v}^{o}|v\in\mathcal{V}\}$.
\end{algorithm}

%\subsection{Dimension Reweighting}
\begin{algorithm}[t]
	\caption{Dimensional Reweighting Convolutional Layer \label{algo:dr}}
	\KwIn{network $(\mathcal{V},\mathcal{E},\mathcal{R}_i)$, $\mathcal{V}$ set of nodes (in batch),$\mathcal{E}$ set of edges, $\mathcal{R}_i=\{\mathbf{r}^{i}_v|v\in \mathcal{V}\}$ set of input representations.  }
	\KwOut{set of output representations $\mathcal{R}_o$ }
	Calculate a dimension scalar $\mathbf{s}$ using $\mathcal{R}_i$.
	
	\ForEach {$v\in\mathcal{V}$}{
	Compute reweighted node representations $\mathbf{r}^{r}_{v}=\mathbf{s}*\mathbf{r}^{i}_{v}$
	}
	\ForEach{$v\in \mathcal{V}$}{
	    Sample neighborhood $N_v\subseteq \mathcal{N}_v$\\
        Aggregate node representations of $N_v$ for node $v$ 
        $\mathbf{r}^{a}_v=a(\mathbf{r}^{r}_{t}|t\in N_v\cup \{v\})$\\
	    Use a neural network layer to transform $\mathbf{r}^{a}_v$ to output representation $\mathbf{r}_{v}^{o}$,      $\mathbf{r}_{v}^{o}=f(\mathbf{r}^{a}_{v})$ (Typically $f(\mathbf{x})=\sigma(\mathbf{W}\mathbf{x}+\mathbf{b})$)
	}
	Output $\mathcal{R}_{o}=\{\mathbf{r}_{v}^{o}|v\in\mathcal{V}\}$.
\end{algorithm}



